Severe flooding and cause-specific hospitalization in the United States

Flooding is one of the most disruptive and costliest climate-related disasters and presents an escalating threat to population health due to climate change and urbanization patterns. Previous studies have investigated the consequences of flood exposures on only a handful of health outcomes and focus on a single flood event or affected region. To address this gap, we conducted a nationwide, multi-decade analysis of the impacts of severe floods on a wide range of health outcomes in the United States by linking a novel satellite-based high-resolution flood exposure database with Medicare cause-specific hospitalization records over the period 2000- 2016. Using a self-matched study design with a distributed lag model, we examined how cause-specific hospitalization rates deviate from expected rates during and up to four weeks after severe flood exposure. Our results revealed that risk of hospitalization was consistently elevated during and for at least four weeks following severe flood exposure for nervous system diseases (3.5 %; 95 % confidence interval [CI]: 0.6 %, 6.4 %), skin and subcutaneous tissue diseases (3.4 %; 95 % CI: 0.3 %, 6.7 %), and injury and poisoning (1.5 %; 95 % CI: -0.07 %, 3.2 %). Increases in hospitalization rate for these causes, musculoskeletal system diseases, and mental health-related impacts varied based on proportion of Black residents in each ZIP Code. Our findings demonstrate the need for targeted preparedness strategies for hospital personnel before, during, and after severe flooding.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


